Masked Video and Body-worn IMU Autoencoder for Egocentric Action Recognition

Compared with visual signals, Inertial Measurement Units (IMUs) placed on human limbs can capture accurate motion signals while being robust to lighting variation and occlusion. While these characteristics are intuitively valuable to help egocentric action recognition, the potential of IMUs remains under-explored. In this work, we present a novel method for action recognition that integrates motion data from body-worn IMUs with egocentric video. Due to the scarcity of labeled multimodal data, we design an MAE-based self-supervised pretraining method, obtaining strong multi-modal representations via modeling the natural correlation between visual and motion signals. To model the complex relation of multiple IMU devices placed across the body, we exploit the collaborative dynamics in multiple IMU devices and propose to embed the relative motion features of human joints into a graph structure. Experiments show our method can achieve state-of-the-art performance on multiple public datasets. The effectiveness of our MAE-based pretraining and graph-based IMU modeling are further validated by experiments in more challenging scenarios, including partially missing IMU devices and video quality corruption, promoting more flexible usages in the real world.

==> Tables/cross_dataset.tex <==
\begin{table}[]
\centering
\caption{cross dataset pretraining and finetuning.}
\scalebox{0.9}{
\begin{tabular}{ccccc}
\hline
                 & Modality  & Pretrain & $W\rightarrow C$ & $C\rightarrow W$ \\ \hline
LIMU-BERT{[}3{]} & IMU       & $\xmark$        & 0            & 0            \\
LIMU-BERT{[}3{]} & IMU       & $\cmark$        & 0            & 0            \\
Our EM-MAE       & IMU       & $\times$        & 27.36        & 94.78        \\
Our EM-MAE       & IMU       & $\checkmark$        & 28.08        & 95.21        \\
Our EM-MAE       & Video     & $\times$        & 69.82        & 96.34        \\
Our EM-MAE       & Video     & $\checkmark$        & 82.32        & 98.32        \\
Our EM-MAE       & IMU-Video & $\times$        & 73.19        & 99.47        \\
Our EM-MAE       & IMU-Video & $\checkmark$        & 85.67        & 99.69        \\ \hline
\end{tabular}
}
\end{table}

==> Tex/1-introduction-0222.tex <==


\section{Introduction}
\label{sec:intro}

\begin{figure}[t]
  \centering
   \includegraphics[width=1.0\linewidth]{Figures_img/teasor0218.png}
   % \vspace{-2em}
   \caption{
   Overview of our EgoMotionMAE (EM-MAE). In the pretraining phase, we construct a graph with IMU features and mask some of the feature nodes in the graph and pixel patches in the ego video. The encoder operates on visible nodes and patches, and the decoder tries to reconstruct the original input. In the finetuning and evaluation phase, we propose a challenge of IMU device missing for more flexible usages. Our EM-MAE takes ego video as optional input. It can work with solely IMU modality for user's privacy concerns.
   }
   \label{fig:teasor}
   % \vspace{-1.5em}
\end{figure}

% Video-IMU egocentric action recognition intuitive introduction
The human brain excels at processing information from different senses simultaneously, such as seeing and hearing through the \textit{head}, and feeling movement and touch through the \textit{limbs}. This ability is what researchers in egocentric action recognition aim to replicate. However, previous studies have mostly focused on using video and audio for action recognition. In this paper, we investigate combining egocentric video from the head with motion data from IMUs attached to the limbs, aiming to leverage the strengths of both modalities and provide complementary and comprehensive insights into human actions.

% What is IMU and what is the importance and merit of IMU modality
% (However, our method is not fast at all)
An Inertial Measurement Unit (IMU) is a motion sensor that integrates accelerometers, gyroscopes, and magnetometers to capture sensor acceleration, angular velocity, and orientation. When affixed to human limbs, IMUs are capable of accurately recording human movements. Unlike visual-based methods, IMU signals offer the advantage of preserving user privacy while reducing the need for computational power and storage capacity. Additionally, IMUs exhibit inherent resilience to common visual modality challenges such as occlusions, varying perspectives, changes in lighting, and background distractions. This resilience makes IMUs an invaluable tool for analyzing human actions.


% Challenge 1: IMUs cannot identify objects and surroundings, so videos are necessary
If action recognition depends solely on IMUs, the primary challenge is their inability to recognize specific objects and contextual details in a scene. For instance, distinguishing between actions such as `washing hands' and `washing tomatoes' becomes challenging when only motion data are analyzed. Therefore, we focus on developing a multimodal method to integrate egocentric video information with IMU signals to encompass both the physical movements of the individual and their interactions with their surroundings.

% Challenge 2: The scale of Ego-video-IMU dataset is limited, so self-supervised training is necessary
Another challenge in advancing ego video and body-worn IMU-based action recognition is the limited scale of datasets containing synchronized data across both modalities. CMU-MMAC dataset [] contains both modalities but we discover that only 10\% of the duration has been annotated for actions, with the remaining 90\% of the time involving actions outside of predefined action categories or purposeless movements. Inspired by this, we aim to fully leverage the larger volume of unlabeled data through self-supervised learning. This approach serves as pretraining to develop an effective multimodal encoder for downstream action recognition tasks.

% Introduce method 1: Multimodal MAE
Recent multimodal pretraining methods achieves significant strides and the Masked Autoencoder (MAE) stands out for its ability to integrate and learn from different modalities, such as semantically related image and language [1,2], and synchronized audio and visual data [3,4]. MAE learns a meaningful representation with the pretext task of recovering the original inputs or features from the corrupted ones. With multimodal input, MAE learns a joint representation that fuses the unimodal signals and reconstruct each modality with the joint representation. As shown in \cref{fig:teasor}, we attempt to build an MAE to learn the natural alignment between synchronized video and motion modalities, as well as their mutual completion within and between modalities. 

% Introduce method 2: IMU Graph Motivation
The use of visual modalities for pretraining and action recognition [1,2,3,4] is widely practiced. In our study, we introduce a Masked Autoencoder tailored for IMU sensors attached to human limbs. Drawing inspiration from action recognition models that utilize human pose [5,6,7], where the \textit{relative positions} of human joints are represented as a graph to effectively capture motion patterns for improved action analysis, we assert that IMU sensors on human limbs reflect the \textit{relative motion} of these joints. Consequently, we propose to construct a graph using IMU signal features. 

% Introduce method 2: IMU Graph Merits
The graph structure enables the efficient capture of motion relationships among different IMU sensors. Additionally, IMUs positioned at different parts of the body exhibit distinct correlations with specific actions. For instance, cooking activities are less associated with leg mounted IMUs, whereas exercises involve both arm and leg IMUs. By leveraging the motion relationships, graph neural networks can optimize action recognition.

% Introduce method: overall pretraining
As shown in \cref{fig:teasor}, we employ the GraphMAE [1] approach in the pretraining phase. The IMU signals are transformed to spectrograms and encoded as features to construct the IMU graph. Some of the feature nodes are masked together with egocentric video patches. Our EgoMotionMAE encoder operates on visible nodes and patches, and the decoder tries to reconstruct the original input. In this way, we aim to develop an encoder with a deep understanding of IMU relationships and the intrinsic correlation between body movements and visual perceptions.

% Challenge 3: Real world application - device missing & low light
Considering applying our model in the real world, we design experiments in various challenging scenarios. Regarding the IMU modality, the diversity in user IMU settings poses a significant challenge. Specifically, the number and placement of IMUs may vary across different users or contexts, potentially leading to discrepancies compared with the IMU settings in our training data. We assume to have all the IMU devices for pretraining, and address the challenge of potential device missing in the finetuning and evaluation. In the pretraining phase, we mask some of the node features to simulate the IMU device missing scenario. Because the model is trained to reconstruct the whole IMU graph, it learns to infer global motion patterns from partial data. Regarding the video modality, the visual appearance is significantly affected by ambient lighting, making visual models vulnerable to variations in lighting conditions. Therefore, we employ a sophisticated technique [] to synthesize low-light effects and reduce the signal-to-noise ratio on videos and evaluate our multimodal method. Our method gains an advantage from using IMU features unaffected by visual appearance, leading it to depend more on IMU data in visually challenging scenarios.

% Experiment results
We conduct experiments on two datasets, one in the kitchen cooking scenario [1] and the other in the outdoor exercise scenario [2]. The results show that our EM-MAE model significantly outperforms the performance of baseline models without pretraining or with single-modal pretraining. Furthermore, our experiments confirm the efficacy of constructing the IMU feature graph, regardless of whether pretraining is involved. We also conduct tests under challenging conditions, including finetuning with missing devices, cross-dataset finetuning, and evaluations using synthetic low-light videos. These tests further demonstrate the robustness and adaptability of our model.

% Contributions
In summary, our main contributions are as follows:
\begin{itemize}
% \vspace{-0.8em}
\item{We design a multimodal masked autoencoder that fuses egocentric video and body-worn IMU signals to achieve a more accurate and robust action recognition model.}
% \vspace{-0.8em}
\item{We propose to construct a graph with features of IMUs attached to different body locations and design an MAE-based pretraining method for the IMU modality by reconstructing corrupted IMU features.}
% \vspace{-0.8em}
\item {
Our experiments show that our method outperforms various baseline methods and continues to exhibit robust performance and adaptability in challenging scenarios, including missing IMU devices and low-light videos, for more flexible usages in the real world.}
\end{itemize}

==> Tex/3-method-0222.tex <==
\section{Method}

\subsection{Characteristics of Video and IMU Data}
% videomae 3.2
The egocentric video and IMU modalities possess distinct characteristics and advantages, which motivate our design of EgoMotionMAE.

\noindent 1. \textbf{Ego video and IMU signals are complimentary.} Egocentric video captures the dynamic appearance of objects and surroundings, yet it contains significant temporal redundancy and correlation []. In contrast, IMU signals directly focus on the subject's movements, closely aligning with the actions' verbs, but they fall short in providing insights into the subject's surrounding context. Thus, the challenge lies in how to fuse these two modalities to enhance accuracy and robustness.

\noindent 2. \textbf{Video and IMU signals are correlated.} Firstly, in egocentric videos, the movements of visible upper limbs show a strong correlation with the IMU signals from the devices attached to these limbs. Secondly, the movement captured by the head-mounted camera is closely related to the IMU signals from the subject's lower limbs. Previous research [] also highlights the potential of using egocentric videos to deduce the movements of a subject's legs. Therefore, there exists significant potential in investigating the synergistic alignment and enhancement during pretraining.

\noindent 3. \textbf{Multiple IMU devices are collaborative.} IMU devices positioned at various locations on the human body collect complementary data, providing a holistic perspective on body movements. However, their contributions to action recognition are not always equal. Thus, our goal is to develop a method that efficiently captures the motion relationships between different IMU devices to enhance action recognition.


\subsection{Masked Autoencoders Preliminaries}
% videomae 3.1 and ICCV23 audio-video mae 3.1

Inspired by video and audio-based MAE methods, our method is also designed based on the operational logic of imageMAE. 
In imageMAE, the input image $D_{im}$ is tokenized to $T_{im}$ in accordance with the setup of prior supervised learning methods using transformers, by conducting a linear projection of non-overlapping patches. 
Positional embeddings $P_{im}$ are then appended to each patch. 
Subsequently, a random subset of these tokens $TM_{im}$ is masked, and only the unmasked tokens $TU_{im}$ are forwarded to the transformer encoder with learnable mask tokens. 
In the final step, a transformer decoder is employed to attempt the reconstruction of the original image $D_{im}$ in pixel space, utilizing the mean squared error (MSE) as the loss function.

\subsection{Problem definition}

We use a 2-second clip of synchronized video and IMU signals as input for pretraining and finetuning the model. The video can be represented as $D_v \in ...$. For the IMU data, we consider four IMU sensors installed on the person's left and right wrists and left and right feet. For each IMU, we read the acceleration in the $x$, $y$, and $z$ axes. Overall, the IMU signals can be represented as $D_{rawIMU} \in ...$. We also consider challenges in real-world scenarios, including finetuning with a less number of IMU devices and evaluation with low-light videos. We aim to design a model to address these challenges without modifying model structure. The experiment settings are detailed in Section 4.x.

\subsection{Patchification and masking}

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{1.2in} \rule{1.0\linewidth}{0pt}}
   % \includegraphics[width=1.0\linewidth]{Figures/teaser2.pdf}
   % \vspace{-2em}
   \caption{
   Patchify and masking.
   }
   \label{fig:patch_mask}
   % \vspace{-1.5em}
\end{figure}

% Patch
As shown in \cref{fig:patch_mask}, the preprocessing of each 2-second raw IMU signal involves several steps. First, the cleaning phase identifies and interpolates missing or NaN values. In the normalization and resampling phase, due to varying sample rates across IMU sensors, signals are resampled to a consistent rate and normalized to a uniform value range in preparation for Fourier transformation. The STFT (Short Time Fourier Transform) step then processes the 1D acceleration signal, converting it into a sequence of 128-dimensional features, resulting in a 320(time) × 128(frequency) spectrogram. This spectrogram is subsequently divided into 160 square patches of size 16 × 16, which serve as the input for the model. For the egocentric video, we follow videoMAE [], where each 2-second video segment is downsampled to 16 frames and then divided into 16 × 16 square patches.

For the IMU spectrograms, we employ unstructured random masking with a masking ratio of 0.75 and also report the performance of structured masking in Section 4.x, including randomly masking a portion of time and frequency of the IMU spectrogram. For videos, we employ the tube masking strategy with a high masking ratio 0.9 [], where the masking map is the same for all frames.


\subsubsection{3.3.3 Network structure}

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{1.8in} \rule{1.0\linewidth}{0pt}}
   % \includegraphics[width=1.0\linewidth]{Figures/teaser2.pdf}
   % \vspace{-2em}
   \caption{
   Network
   }
   \label{fig:network}
   % \vspace{-1.5em}
\end{figure}

We use the standard Transformer (Vaswani et al., 2017) as our main model component. Each Transformer layer consists of multi-headed self-attention (MSA), layer normalization (LN), and multilayer perceptron (MLP) blocks with residual connections. Specifically, we denote a Transformer layer y = Transformer(x; MSA, LN1, LN2, MLP) as: x ′ = MSA(LN 1 (x)) + x; y = MLP(LN 2 (x ′ )) + x ′, where MSA computes dot-product attention of each element of x and thus has a quadratic complexity w.r.t. to the size of x.

% videomae 3.3
Backbone: joint space-time attention.

% MAE that listen Encoder. 
Audio-MAE uses a stack of standard Transformers [2] as its encoder. The encoder only processes (20\%) non-masked patches to reduce computation overhead which is quadratic to the input sequence length. We use the 12-layer ViT-Base (ViT-B) [9] Transformer as our default.

% MAE listen Spectrogram Patch Embeddings.
Following [10, 18], we transform audio recordings into Melspectrograms and divide them into non-overlapped regular grid patches. These patches are then ﬂattened and embedded by a linear projection. Similar to MAE [1], we add ﬁxed sinusoidal positional embeddings to the embedded patches. 

graph encoder

graph decoder


\subsubsection{3.3.4 Pretraining criterion}

% pixel reconstruction

% Graph feature reconstruction

\subsubsection{3.3.5 Finetuning for action recognition}

% MAE that listen Fine-tuning for Downstream Tasks. 
In the ﬁne-tuning stage, we only keep and ﬁne-tune the AudioMAE encoder and discard the decoder. Different from the original MAE, and inspired by [47, 28], we also explore to employ masking in the ﬁne-tuning stage to remove a portion of patches to further regularize learning from a limited view of spectrogram inputs, which, as a side effect, also reduces computation during ﬁne-tuning. Compared to SpecAug [48] which takes full-length input with the masked portion set to zero as data augmentation, Audio-MAE sees only a subset of real-valued input patches without the nulliﬁed ones. Audio-MAE then encodes these non-masked patches and applies an average pooling layer followed by a linear layer on top for ﬁne-tuning in classiﬁcation tasks.

\subsubsection{3.3.6 Implementation details}

% loss weight

\clearpage

==> Tex/variable_names.tex <==
$T$ (2s) time
$c$ (32 and 18) class number


$D_v \in \mathbb{R}^{T \times S_v \times H \times W \times 3}$ video
$S_v$ (30fps) video sample rate
$t_v$ (16 frames/ 2 seconds) downsampled frames number
$p_v$ (1536) video square patches of size 16 x 16



$S_i$ IMU sample rate
$N_i$ (4) the number of IMUs
$D_{ri} \in \mathbb{R}^{N_i \times T \times S_i \times 3}$ raw IMU
$t_i$ (160) resampled temporal points IMU
$d_i$ (128) dimensions IMU feature
$D_{si} \in \mathbb{R}^{t_i \times d_i}$ IMU spectrogram
$p_i$ (80) IMU square patches of size 16 × 16 in one spectrogram
